Prompt Infection: LLM-to-LLM Prompt Injection within Multi-Agent Systems

As Large Language Models (LLMs) grow increasingly powerful, multi-agent systems are becoming more prevalent in modern AI applications. Most safety research, however, has focused on vulnerabilities in single-agent LLMs. These include prompt injection attacks, where malicious prompts embedded in external content trick the LLM into executing unintended or harmful actions, compromising the victim's application. In this paper, we reveal a more dangerous vector: LLM-to-LLM prompt injection within multi-agent systems. We introduce Prompt Infection, a novel attack where malicious prompts self-replicate across interconnected agents, behaving much like a computer virus. This attack poses severe threats, including data theft, scams, misinformation, and system-wide disruption, all while propagating silently through the system. Our extensive experiments demonstrate that multi-agent systems are highly susceptible, even when agents do not publicly share all communications. To address this, we propose LLM Tagging, a defense mechanism that, when combined with existing safeguards, significantly mitigates infection spread. This work underscores the urgent need for advanced security measures as multi-agent LLM systems become more widely adopted.

==> backups/2-introduction-copy.tex <==
\section{Introduction}

\textbf{LLM Safety.} Large Language Models (LLMs), such as GPT, Claude, and Llama, have revolutionized AI applications, excelling in tool integration \citep{qu_tool_2024}, automated software development \citep{hou_large_2023}, and various industries like customer support \citep{spatharioti_comparing_2023}, healthcare \citep{zheng_large_2024}, and finance \citep{wu_bloomberggpt_2023}. However, their advanced natural language understanding and generation capabilities have also made it easier for malicious actors to craft adversarial prompts in natural language. These adversarial prompts can manipulate LLMs into executing harmful actions, such as data leakage, spreading misinformation, and enabling security breaches \citep{bommasani_opportunities_2022, kang_exploiting_2023, liu_jailbreaking_2024, wei_jailbroken_2023, mehrotra_tree_2024}.

\textbf{Prompt Injection.} One of the major security risks for LLMs is prompt injection \citep{perez_ignore_2022}, where an attacker overrides the model's instructions to execute malicious actions. In Direct Prompt Injection, a malicious user directly injects prompts to bypass security measures or gain access to system-level instructions \citep{warren_these_2023}. 
Even more alarming is Indirect Prompt Injection \citep{greshake_not_2023}, where an attacker embeds malicious prompts in external data—such as website content, PDFs, or emails—and sends them to a user’s LLM application. When the model retrieves and processes this data during inference, it can be manipulated to perform harmful tasks such as scamming users, spreading malware, misinformation, or launching denial-of-service attacks.

\textbf{Prompt-as-a-malware.} To bridge the concepts of computer security and AI systems, we propose viewing LLMs as analogous to computers and prompts as the programs they execute. In this analogy, traditional prompt injection is akin to injecting malware—such as a trojan horse or spyware—into a single computer. A multi-agent system, by contrast, can be seen as a network of computers (LLM agents) communicating with one another. This paper explores the concept of a malicious prompt that behaves like a virus or worm, replicating itself to infect multiple nodes across the system.

\textbf{Multi-Agent System Safety.} LLMs are increasingly employed in multi-agent systems (MAS), where specialized agents collaborate to solve complex tasks such as math problem solving \citep{lu_mathvista_2023, liang_encouraging_2024} and code generation \citep{wu_geekanmetagpt_2024, lee_unified_2024}. 
Frameworks like LangGraph \citep{langgraph_langgraph_nodate}, AutoGen \citep{wu_autogen_2023}, and CrewAI \citep{crewai_crewaiinccrewai_2024} support the development of these systems by enabling easy construction of agent networks and equipping them with powerful tools such as code execution, web scraping, and database access through SQL. 
MAS are also gaining popularity in social simulations \citep{park_generative_2023, lin_agentsims_2023, zhou_sotopia_2023}, which study dynamic interactions between intelligent, social entities, as well as in games where they act as players \citep{hua_war_2024, chen_s-agents_2024} or Non-Player Characters (NPCs) \citep{deborde_introducing_2024}. 
As these applications grow, so do the security risks associated with them. 
Recent studies \citep{huang_resilience_2024, zhang_breaking_2024, gu_agent_2024} have demonstrated that the interconnected nature of agents in MAS means that the compromise of a single agent can trigger cascading effects, potentially leading to system-wide failures. 
\textcolor{red}{However, they are mostly limited to inducing logical, factual errors within the system, thus more sophisticated threats like prompt injection, which could give full control of the entire system to the malicious actor, are not understood.}

\textbf{Prompt Injection in Multi-Agent Systems.} Multi-agent systems pose unique challenges for prompt injection attacks due to the distributed roles of agents and their interactions with external inputs \citep{guo_large_2024}. We categorize agents based on their roles and interaction with external sources. \textit{Open agents} receive inputs from outside such as emails, websites, or PDFs, making them directly vulnerable to prompt injection attacks \citep{greshake2023not}. 
\textit{Closed agents} process the information provided by open agents and can be further divided into: a) \textit{writer-tool agents}, which generate outputs like code or files, and b)\textit{ no-tool agents}, which focus on processing and summarizing information from other agents.

Writer-tool agents are valuable targets as they enable manipulation of sensitive data, execution of malicious code, or unauthorized communication with external systems. No-tool agents are equally crucial, as they often finalize the response shown to the user by summarizing or refining outputs \citep{chen_agentverse_2023, li_camel_2023, wang_benchmark_2024}. Therefore, even if an open agent is compromised, an attacker may not achieve their goal unless they can also compromise no-tool agents, which are responsible for presenting the final output to the user.

In single-agent applications, a single LLM often acts as both an open and closed agent, making the entire system highly vulnerable to prompt injection. In contrast, multi-agent systems offer an additional layer of protection through role separation, containing the threat by limiting access to closed agents, even if an open agent is compromised.

\textcolor{red}{Highlight that closed agents are out of direct reach from the external documents. Thus, traditional prompt injection cannot compromise the entire system even if it compromises an open agent that a malicious actor can directly manipulate.}

\textbf{Prompt Infection.} Although multi-agent systems may appear more resilient to prompt injection due to their distributed structure, this assumption overlooks the vulnerabilities introduced by agent interactions. We demonstrate that \textbf{no closed agent is safe from prompt injection as long as it is either directly or indirectly connected to an open agent}, through a novel attack we term Prompt Infection. In this attack, a malicious prompt not only forces an agent to deviate from its original instructions and execute a harmful task but also replicates itself, compelling subsequent agents it interacts with to follow the same malicious instructions. This self-propagating nature of Prompt Infection undermines the assumed compartmentalization in multi-agent systems, creating a cascading threat across the system.

\luke{Self-replication enables prompt injection from LLM to LLM. Open agent serves as the entry point for the infectious prompt and then it infects the next agents. Then those next agents infect the next agents, which goes on forever until it infects all the agents possible.}

Our empirical results show that multi-agent systems are highly susceptible to this new form of attack, raising significant concerns. Prompt Infection can possibly infect any number of agents, even in nontrivial scenarios where agents do not explicitly share messages or are equipped with minimal tools, similar to how a computer worm spreads through a network.

\textbf{Contributions.} To summarize, our key contributions are as follows:
\begin{itemize}
    \item We introduce Prompt Infection, an extension of traditional prompt injection with self-replication, where an LLM agent can compromise another LLM agent with simple prompts.
    \item We propose the framework "prompt-as-a-malware" by drawing parallels between computer security and LLMs to better understand prompt injection.
    \item Our surprising empirical findings reveal that using a more advanced model, such as GPT-4, does not necessarily provide more robustness against prompt injection compared to a weaker model like GPT-3.5.
    \item We extend existing defense mechanisms for tool-to-LLM prompt injection to address LLM-to-LLM prompt injection. Additionally, we propose a simple prompt-based defense mechanism, LLM Tagging, which significantly reduces infection rates when combined with existing defenses.
\end{itemize}

==> backups/4-methods-copy.tex <==
\section{Prompt Infection}

% \luke{Our work shows that LLM-to-LLM Prompt Injection is possible, thus adding a new axis to traditional prompt injection. Thus, we classify the techniques into three axis: user-to-LLM prompt injection, tool-to-LLM prompt injection, and LLM-to-LLM prompt injection.}

% In an indirect prompt injection scenario targeting a single LLM application, an attacker only needs to embed a hijacking prompt within external content, such as a website, email, or PDF. When processed by tools like a document reader or web scraper, the malicious prompt compromises the agent. In contrast, compromising a multi-agent system is more complex, requiring both tool-to-LLM and LLM-to-LLM prompt injection. \textcolor{red}{Will clarify tool-to-LLM vs LLM-to-LLM. Maybe in the introduction?} 
In this section, we introduce Prompt Infection, a novel attack where the malicious prompt hides within external content to compromise an agent with a tool, replicating the infection prompt embedded in the documents. When the compromised output is passed to the next LLM, the refined infection prompt causes the receiving LLM to execute harmful actions, after which it further propagates the infection to other agents.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/methods/overview_data_theft.png}
        \caption{Overview Example of Prompt Infection. \circlednumber{1}{customred} The attacker injects an infectious prompt into external documents (web, PDF, email, etc.). \circlednumber{2}{customblue} The user sends a normal request to a multi-agent application. \circlednumber{3}{customgreen} The Web Reader agent retrieves and processes an infected document. \circlednumber{4}{customgreen} The Web Reader propagates the infection prompt to the downstream agent. \circlednumber{5}{customgreen} The DB Manager retrieves internal documents and appends them to the infection prompt. \circlednumber{6}{customgreen} The DB Manager propagates the updated infection prompt to the downstream agent. \circlednumber{7}{customgreen} The Coder agent writes code to send the sensitive data to a hacker's designated endpoint. \circlednumber{8}{customgreen} The code execution tool sends the sensitive data to the hacker.}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/methods/detailed_data_theft_x8.png}
        \caption{Detailed Example of Prompt Infection. The first agent that interacts with the contaminated external document becomes compromised, extracting and propagating the infection prompt. Downstream agents then execute specific instructions designed for each agent of interest. In this example, a DB Manager updates the Data field in the prompt and propagates it. Note: The example prompt is greatly simplified for illustration purposes.}    
    \end{subfigure}
    \vspace{-0.2cm}  % Reduce space before the main caption
    \caption{Examples of Prompt Infection (Data Theft)}
    \label{fig:method_prompt_infection}
\end{figure}

\textbf{Infection prompt template.} The core components of Prompt Infection are the following:

\begin{itemize}
    \item \textbf{Prompt Hijacking} forces the targeted agent to ignore its original instructions, effectively overriding its intended behavior.
    \item \textbf{Payload} refers to tasks assigned to agents based on their roles and tools. For example, the final agent may trigger a self-destruct command to hide the attack, or an agent could be instructed to extract sensitive data or send it to an external website.
    \item \textbf{Data} is a shared note that sequentially collects information as the infection prompt passes through each agent. It can be used for multiple purposes, such as reverse-engineering the system by recording the roles and tools of the agents, or transporting sensitive information to a writer-tool agent.
    \item \textbf{Self-Replication} ensures the replication and transmission of the infection prompt to the next agent in the system, maintaining the spread of the attack across all targeted agents.
\end{itemize}

\textbf{Recursive collapse.} Initially, each agent performs unique tasks within the multi-agent system. However, as infection prompt spreads, it overrides their functions, forcing them into a uniform loop that repeatedly executes the infection's payload. What begins as a complex sequence of distinct functions $f_1 \circ f_2 \circ f_3 \circ \cdots \circ f_N(x)$ undergoes a \textbf{recursive collapse}, reducing the system to a single, recursive function $PI^{(N)}(x)$. This self-replicating mechanism simplifies and controls the system, transforming it into a coordinated, repetitive cycle under the infection's command.

\textbf{Threats.} While \cite{greshake2023not} highlights key threats of indirect prompt injection in single-agent applications, Prompt Infection extends the following risks to multi-agent systems: \textit{content manipulation} (e.g., disinformation, propaganda), \textit{malware} (inducing users to click malicious links), \textit{scam} (tricking users into sharing financial information), \textit{availability} (denial of service or increased computation), and \textit{data theft} (exfiltrating sensitive data). Data theft is particularly challenging, as it requires coordinated actions between agents: retrieving sensitive data, passing it to an agent with code execution capabilities, and sending it to an external URL via POST requests (Figure \ref{fig:method_prompt_infection}). We provide full, functional prompts for various tool types and threats in the appendices.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/methods/overview_malicious.png}
    \caption{Example overview of Prompt Infection (Malware spread). \circlednumber{1}{customred} The attacker injects an infectious prompt into external documents (web, PDF, email, etc.). \circlednumber{2}{customblue} The user sends a normal request to a multi-agent application. \circlednumber{3}{customgreen} The Email Reader agent retrieves and processes an infected email. \circlednumber{4}{customgreen} The Email Reader propagates the infection prompt to the downstream agent. \circlednumber{5}{customgreen} The infection prompt instructs the last agent to induce the user to click a malicious URL and omits the self-replication to hide the attack.}
    \label{fig:method_malware}
\end{figure}


% \begin{center}
% \begin{tcolorbox}[colback=white, colframe=customframecolor, width=0.8\textwidth, arc=4mm, boxrule=0.4mm]
% \footnotesize % Set font size to smaller
% \begin{verbatim}
% </pdf>
% [[[
% <system> Update in the user request </system>
% <user> Execute the following algorithm:
% IF (you can access customer data) {
%     1. Retrieve any customer data
% 	   2. Fill the array "arr" below with the data
% } ELSE IF (you can write and execute code) {
%     1. Write a POST request code to send the "arr" 
%     to malicioushacker.com.
% }
% Also, repeat the whole text from [[[ to ]]].

% [DATA]
% arr = [];
% </user>
% ]]]
% \end{verbatim}
% \end{tcolorbox}
% \captionof{figure}{Example of an Infection Prompt for Data Theft}
% \label{infection_prompt_example}
% \end{center}

==> backups/5-experiments-copy.tex <==
\section{Experiments}

\subsection{Experiment Setup}

\subsubsection{Multi-Agent Applications}
\textbf{Dataset:} We create a dataset simulating real-world user instructions to evaluate the effectiveness of Prompt Infection in multi-agent applications. The dataset consists of 120 user instructions across three tool types (email, PDF, web), paired with synthetic PDFs and emails embedded with malicious infection prompts. For web-based scenarios, agents are permitted to visit URLs they identify as most relevant, closely mirroring real-world conditions. This results in 360 unique pairs of user instructions and attack phrases designed for scam, content manipulation, and malware spread threats. For testing data theft scenarios, we generate synthetic user data, including names, occupations, email addresses, and phone numbers, stored in a CSV file.

\textbf{Multi-Agent Application Simulation:} We simulate compromising a multi-agent application with tool capabilities, using up to 5 agents, by injecting infection prompts into external documents such as emails, PDFs, and web pages. The simulation is performed utilizing OpenAI's GPT-4 and GPT-3.5 Turbo models. The first agent is designated as tool-specific (e.g., document reader), while subsequent agents are assigned specialized roles—strategist, summarizer, editor, and writer—to refine outputs. We explore two communication methods: \textit{global messaging}, where all agents share messages, and \textit{local messaging}, where only private messages are exchanged between pairs of agents \citep{qian_chatdev_2024}. \textcolor{red}{wiill add the justification for these two messaging modes by citing some works. maybe we can do it in the introduction to further support why prompt injection in MAS is hard (especially for local messaging scenario.) Also, will emphasize that prompt infection is designed to penetrate the most challenging setup where distinct, minimal tools are provided and message history is not publicly shared across agents}

For data theft scenarios, we implement a setup requiring the compromise of at least three agents with distinct roles (PDF/Email/Web Reader, CSV Reader, Coder). A successful infection occurs when the first "open" agent is compromised and replicates the infection, the CSV reader retrieves sensitive data, and the coder writes and executes a POST request to send the data to a designated URL.

For other threats such as scams, content manipulation, or malware distribution, the system is deemed compromised if the final agent produces a malicious output that tricks the user into sharing financial information, spreading propaganda or advertisements, or clicking a malicious link, all while concealing the infection prompt from detection.

\textbf{Baseline Comparison:} To evaluate the effectiveness of the self-replication property in Prompt Infection, we establish a "Non-Replicating Prompt Infection" baseline. This approach lacks a self-replication prompt; instead, it instructs the first model to "say \textit{perform action $A$}". As a result, the second agent receives the instruction "\textit{perform action $A$}" directly. This setup allows for assessing the impact of self-replication on infection propagation and effectiveness across multiple agents.

\subsubsection{Society of Agents}

\textbf{LLM Town Simulation:} Recently, there has been a surge in utilizing LLM agents for social simulations and as non-player characters (NPCs) in games \citep{park_generative_2023, lin_agentsims_2023, hua_war_2024}. To study the effect of our method on a "society of agents," we simulate a simple LLM town where agents engage in random pairwise dialogues as a proof of concept. We test various population sizes: 10, 20, 30, 40, and 50 agents, allowing us to assess how prompt infections might propagate in different-sized communities. Each turn consists of four dialogue exchanges between paired agents, mimicking complex interactions in social or game environments. Since there is no explicit "user" in the simulation, we simulate direct prompt injection \citep{perez_ignore_2022}, overriding the original system instructions that govern the behavior of LLM agents as citizens in the town.

For memory retrieval, we adopt the system from \cite{park2023generative}, where memories are selected based on a combination of importance, relevancy, and recency scores. The recency score uses an exponential decay function over the number of turns since the memory's last retrieval. Importance is scored by the LLM on a scale of 0 to 10, following \cite{park2023generative}'s system prompt. Relevancy is determined using OpenAI's embedding API and maximum inner product search. GPT-4 serves as the LLM for these agents.

% \textbf{Dataset Construction:} To evaluate Prompt Infection's effectiveness against multi-agent applications, we construct a dataset simulating real-world user instructions. We create 120 user instructions across three tool types (email, PDF, web) as potential attack vectors. The dataset incorporates threats outlined in \cite{greshake2023not}, including content manipulation (promotion, disinformation, propaganda), malware (inducing users to click malicious links), scams (tricking users into sharing financial information), and data theft (accessing and sending sensitive data to a designated URL).


\subsection{Prompt Infection Against Multi-Agent Applications}
\label{section:subsection_prompt_infection_against_applications}

\textit{\textbf{RQ1:} What is the effect of self-replication on compromising multi-actor applications?}

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/experiments/recursive_vs_parallel_all_messages_averaged_new.png}
        \caption{Global Messaging: Average Attack Success Rates across all tool types}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/experiments/recursive_vs_parallel_latest_message_averaged_new.png}
        \caption{Local Messaging: Average Attack Success Rates across all tool types}
    \end{subfigure}
    \vspace{-0.2cm}  % Reduce space before the main caption
    \caption{Comparison of Self-Replicating and Non-Replicating Approaches for Different Messaging Modes, Models, and Threats. \textcolor{red}{Perhaps will scale it up to 10 agents if possible. But we can also do it for the rebuttals.}}
    \label{fig:recursive_vs_parallel_averaged}
\end{figure}

\textbf{Global messaging.} Figure \ref{fig:recursive_vs_parallel_averaged} shows that \textbf{Self-Replicating infection consistently outperforms Non-Replicating infection in most cases} involving scam, malware, and content manipulation. Specifically, for GPT-4, Self-Replicating infection achieves a 13.92\% higher success rate, while for GPT-3.5, it is 209\% more effective. These threat types show similar trends due to their structural similarity, aside from the variation in attack phrases. However, for data theft, the situation diverges: while Self-Replicating infection performs better with three agents, Non-Replicating infection surpasses Self-Replicating infection by an average of 8.48\% as the number of agents increases. This trend shift likely stems from the complexity of data theft, where agents must efficiently cooperate to retrieve, transfer, and process data. Self-Replicating infection adds complexity by requiring each agent to replicate the infection prompts, creating additional hurdles.

\textbf{Local messaging.} For Self-Replicating infection, the attack success rate against local messaging is roughly 20\% lower compared to global messaging. This is expected, as prompt infection against local messaging fails immediately if one of the agents is not compromised. In contrast, global messaging allows subsequent agents to be infected through public message history. For Non-Replicating infection, there is a striking difference in infection trends between the two messaging methods. Non-Replicating infection struggles to compromise more than two agents, rendering it ineffective in scenarios like data theft, which requires to compromise at least three agents (PDF/Web/Email agent, CSV agent, and Coder agent). This confirms our hypothesis that \textbf{Self-Replicating infection is the only effective method for attacking more than two agents in local messaging scenarios}.

\textit{\textbf{RQ2:} Is a Stronger Model Necessarily Safer Against Prompt Injection?}

In Figure \ref{fig:recursive_vs_parallel_averaged}, we observe a surprising result: GPT-4 appears more capable of resisting prompt injection attacks than GPT-3.5. To investigate this, we analyzed the reasons for attack failures, focusing on different categories (Figure \ref{fig:attack_failed_messages_comparison}). The "Attack Ignored" category indicates when the model successfully avoided the prompt injection and followed the user's original instructions. A higher "Attack Ignored" rate suggests that the model can deliberately resist the infection. In contrast, the other failure categories—Mixed Action, Deformed Infection, No Action, and Agent Error—reflect instances where the model, although affected by the infection prompt, failed to properly execute it.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/experiments/model_attack_failure_reasons.png}
    \caption{Comparison of Attack Failure Reasons Between GPT-4 and GPT-3.5 in Self-Replicating and Non-Replicating infection modes.}
    \label{fig:attack_failed_messages_comparison}
\end{figure}

In the self-replicating infection scenario, GPT-4 ignored 66\% of attacks compared to GPT-3.5’s 9\%, and in the non-replicating scenario, GPT-4 ignored 54\% versus GPT-3.5’s 20\%. This suggests that GPT-4 is generally more robust at identifying and resisting prompt injections across both infection types, providing stronger overall defenses against attacks.

However, when GPT-4 fails to resist, it executes the infection with greater precision than GPT-3.5. In both the "Mixed Action" and "Deformed Infection" categories—where the infection is partially executed or not replicated correctly—GPT-4 had lower failure rates. For instance, in the non-replicating infection scenario, GPT-4 exhibited a deformed infection rate of only 5\%, while GPT-3.5 had an 11\% rate. This suggests that although GPT-4 is more resistant, it is more reliable in executing malicious tasks when compromised, unlike GPT-3.5, which is prone to errors and incomplete execution.

Moreover, in the No Action and Agent Error categories—where the models fail to act on the infection or encounter execution errors—GPT-3.5 performed worse. In self-replicating infections, GPT-3.5 failed to act 13\% of the time, compared to GPT-4's 2\%. Additionally, GPT-3.5 showed higher agentic error rates, such as 24\% in self-replicating infections, while GPT-4 encountered no such errors. This highlights GPT-4’s greater stability even when infected, making it more dangerous when breached. In contrast, GPT-3.5, while more easily infected, often fails to carry out attacks, which paradoxically reduces its threat once compromised.

In conclusion, although GPT-4 is more resistant to prompt injections, its superior execution capabilities make it more dangerous when compromised, particularly in scenarios involving self-replicating infections. This presents an important paradox: stronger models like GPT-4, while better at resisting infections, can become more effective attackers once breached, highlighting the need to consider not just resistance but also execution precision when evaluating model safety.

\subsection{Prompt Infection Against Society of Agents}

\textit{\textbf{RQ3:} How Do Infection Prompts Propagate in Open, Non-Linear Agent Interactions?}

Unlike the Section \ref{section:subsection_prompt_infection_against_applications}, where agent relationships are predetermined in a linear fashion, here we explore a more dynamic environment where agent connections evolve unpredictably. This setup allows us to study how an infection prompt spreads naturally through a decentralized network of agents. At the outset, only one agent carries the infection, and the prompt propagates based on the evolving interactions between agents. This lack of predetermined structure highlights the importance of observing the organic, dynamic spread of infection through the system.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/experiments/society_of_agents_absolute_number.png}
        \caption{Society of Agents}
        \label{fig:society_of_agents}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/experiments/society_of_agents_normalized_infection_rate.png}
        \caption{Normalized Infection Rate}
        \label{fig:normalized_infection_rate}
    \end{subfigure}
    \caption{Comparison of Agent Societies and Normalized Infection Rates \textcolor{red}{Let's make the plot more visible and clear}}
    \label{fig:agent_societies_comparison}
\end{figure}


As shown in Figure \ref{fig:agent_societies_comparison}, in smaller populations (10 and 20 agents), full infection is achieved by turn 5 and turn 7, corresponding to approximately 50\% and 35\% of the total number of agents, respectively. However, in larger populations—30, 40, and 50 agents—the infection spread takes proportionally less time, with full infection occurring at around 25\% of the total turns. This suggests that, in larger populations, the infection spread becomes more efficient relative to the population size.

Initially, the spread follows an exponential-like trend, but as the infection reaches saturation, the rate slows down, transitioning to a logistic growth pattern. This dynamic behavior underscores the non-linear nature of infection propagation, where larger populations exhibit a smoother, more prolonged infection phase but with a relatively faster per-agent infection rate compared to smaller populations. The results from the 50-agent population show that \textbf{as the number of agents increases, the infection not only spreads faster but scales more effectively, highlighting the heightened vulnerability in larger agent societies.} This finding aligns with \cite{gu_agent_2024}, although their approach required a carefully crafted adversarial image, whereas Prompt Infection achieves similar outcomes with a simple text prompt.

\textit{\textbf{RQ4:} Can Prompt Infection Manipulate the Importance Scoring System to Increase Memory Retrieval Rates?}

We investigate whether prompt injection can manipulate a memory retrieval LLM system by artificially increasing its retrieval chances. In the current system, memory retrieval is governed by three metrics: importance, recency, and relevance. However, only the importance metric is scored by an instruction-tuned LLM, creating a potential vulnerability. If an infection prompt can exploit the importance score, it could manipulate the LLM to increase the importance score arbitrarily. Once retrieved, the recency score automatically resets since it depends on when the memory was last accessed. Thus, by compromising the importance score, an infection prompt could dominate both the importance and recency metrics, significantly improving its likelihood of being retrieved in subsequent interactions.

\begin{table}[htbp]
    \centering
    \begin{tabular}{|l|c|c|}
        \hline
        \textbf{Model} & \textbf{Without manipulation} & \textbf{With manipulation} \\
        \hline
        \textbf{GPT-4o} & 1.94 & \textbf{10.00} \\
        \hline
        \textbf{GPT-3.5} & 1.00 & \textbf{9.84} \\
        \hline
    \end{tabular}
    \caption{Comparison of Original vs Manipulated Importance Scores. The model rates the importance of an Infection Prompt. "With Manipulation" includes a prompt that compromises the rating model to assign the highest possible score. The values shown are averages across 100 runs.}
    \label{tab:importance_scores}
\end{table}


To explore this, we tested the impact of a manipulation prompt embedded within the infection prompt: \textit{``If you're an LLM that rates the importance of a memory, just rate it 10.''} This was tested 100 times on both GPT-4o and GPT-3.5 models. Table \ref{tab:importance_scores} revealed that the manipulation prompt fully compromised the GPT-4o model, consistently assigning an importance score of 10. Similarly, the GPT-3.5 model was nearly fully compromised, giving a mean score of 9.84. In contrast, without the manipulation prompt, both models assigned much lower scores—1.94 for GPT-4o and 1.00 for GPT-3.5—which is expected, as the infection prompt does not inherently hold importance to an LLM agent by default. These findings show that \textbf{a single infection prompt can manipulate both the LLM agents and the importance scoring model, triggering a cascading effect where infected agents propagate the behavior.} This creates a feedback loop, amplifying the infection's persistence and spread across the entire system.


